Soteria: Automated IoT Safety and Security Analysis

Broadly defined as the Internet of Things (IoT), the growth of commodity devices that integrate physical processes with digital systems have changed the way we live, play and work. Yet existing IoT platforms cannot evaluate whether an IoT app or environment is safe, secure, and operates correctly. In this paper, we present Soteria, a static analysis system for validating whether an IoT app or IoT environment (collection of apps working in concert) adheres to identified safety, security, and functional properties. Soteria operates in three phases; (a) translation of platform-specific IoT source code into an intermediate representation (IR), (b) extracting a state model from the IR, (c) applying model checking to verify desired properties. We evaluate Soteria on 65 SmartThings market apps through 35 properties and find nine (14%) individual apps violate ten (29%) properties. Further, our study of combined app environments uncovered eleven property violations not exhibited in the isolated apps. Lastly, we demonstrate Soteria on MalIoT, a novel open-source test suite containing 17 apps with 20 unique violations.

==> algo_app_properties.tex <==
\begin{algorithm}[t!]
	\DontPrintSemicolon
	\setstretch{0.9}
    \footnotesize
	\SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
	\DontPrintSemicolon
	\SetNoFillComment % <---------------------------
    %\SetKwInOut{Input}{Input}
    %\SetKwInOut{Output}{Output}
	\Input{$G = \{G_i\}_{i=1}^{n}$: State-models of apps}
	\Output{$Q$: a model for each set of interacting apps}
	\tcc {Acquire devices in states}
	\For{i $\in$ (1:n)}{
		\For{$v \in G_i$}{
			$V_i(v) \gets false$\;
		}%for
	}%for
	\tcc{Construct union (set) of interacting apps}
	\For{i $\in (1:n)$}{
		\While{$\exists$  $v \in G_i$ \normalfont{such that} $V_i(v) = false$}{
			\For{j $\in (1:n)$ where j $\neq$ i}{
				\For{$e \in G_j$}{
					\eIf{$e$ \normalfont{contains} $v$}{
						pick $e$\;
        			 	return\;
      				}%elf.
      				{%else
       				 	$e \gets \emptyset$
      				}%else
				}%For
				%\tcc{Output a model for interacting apps}
				$Q$ $\gets$ a state-model with an initial state\;
                createModel($Q$,  ($v, E^{-}(v)$, i),  ($e, V^{+}(e)$, j))\;
			}%for
			$V_i(v) \gets true$;\
		}%while
	}%for
    \caption{\footnotesize{Finding apps for app-specific properties}}
    \label{algo:app_properties}
\end{algorithm}

==> algo_general_properties.tex <==
\begin{algorithm}[t!]
	\DontPrintSemicolon
	\setstretch{0.9}
    \footnotesize
	\SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
	\DontPrintSemicolon
	\SetNoFillComment % <---------------------------
    %\SetKwInOut{Input}{Input}
    %\SetKwInOut{Output}{Output}
	\Input{$G = \{G_i\}_{i=1}^{n}$ State-models of apps}
	\Output{$Q:$ state model for each set of interacting apps}
	\tcc{Find unique devices in apps}
	\For{i $\in$ (1: n)}{ %for all apps
		$devices \gets \emptyset$\;
		$V$= $V$($G_i$)\;
		\While{$V$ \normalfont{is not empty}}{  
			Pick a vertex $v$ $\in$ $V$\;
			\tcc {d(v): set of device attributes in v}
			%\tcp*{}\; 
			$devices$ $\gets$ $devices$ $\cup$ $d(v)$\;
			$V \gets V \setminus \{v\}$\;
		}%while
	} %for all apps	
	\tcc{Construct union (set) of interacting apps}
	$D$ $\gets$ $devices$\;
	\While{$D$ \normalfont{is not empty}}{
		Pick a device $i \in D$\;
		$Q_i$ $\gets$ a state-model with an initial state\;
	}%while
	\For{i $\in$ (1: n)}{
		\For{j $\in$ (i+1: n)}{
			$remaining$ $\gets$ V($G_i$) $\times$ V($G_j$)\;
				\While{remaining \normalfont{is not empty}}{
					Pick $(v, v') \in remaining$\;
						\For{d $\in$ ($d(v)$ $\cap$ $d(v')$)}{
						   %\tcc{create a model for interacting apps}
							createModel($Q_d$,  ($v, E^{-}(v)$, i),  ($v', E^{-}(v')$, j))\;
						}%for
				}%while
		}%for
	}%for
    \caption{\footnotesize{Finding apps for general properties}}
    \label{algo:general_properties}
\end{algorithm}

